HotStuff-1: Linear Consensus with One-Phase Speculation

This paper introduces HotStuff-1, a BFT consensus protocol that improves the latency of HotStuff-2 by two network hops while maintaining linear communication complexity against faults. Furthermore, HotStuff-1 incorporates an incentive-compatible leader rotation design that motivates leaders to propose transactions promptly. HotStuff-1 achieves a reduction of two network hops by speculatively sending clients early confirmations, after one phase of the protocol. Introducing speculation into streamlined protocols is challenging because, unlike stable-leader protocols, these protocols cannot stop the consensus and recover from failures. Thus, we identify prefix speculation dilemma in the context of streamlined protocols; HotStuff-1 is the first streamlined protocol to resolve it. HotStuff-1 embodies an additional mechanism, slotting, that thwarts delays caused by (1) rationally-incentivized leaders and (2) malicious leaders inclined to sabotage other's progress. The slotting mechanism allows leaders to dynamically drive as many decisions as allowed by network transmission delays before view timers expire, thus mitigating both threats.

==> proof2.tex <==
\section{Correctness Proof of Streamlined HotStuff-1 with slotting}
\label{sec:proof}
In this Section, we prove the \emph{safety} and \emph{liveness} of \PHSOne{} with \emph{slotting}. 
We first prove that no two correct replicas will execute two different requests for the same slot of the same view.

\begin{lemma}\label{prop2:non_divergent}
Let $\Replica_i$, $i \in \{1, 2\}$,  be two correct replicas that executed blocks 
$B_{s,v}^{i}$ for a given view $v$. If $\n = 3\f+1$, then $B_{s,v}^{1} = B_{s,v}^{2}$.
\end{lemma}

\begin{proof}
Similar to the proof of Lemma~\ref{prop:non_divergent}.
\end{proof}


\begin{lemma} \label{lm2:no-gap-rule}
    If block $B_{s,v}$ is directly extended by block $B_{s+1,v}$ and no-gap-extension certificates 
    $\Certificate{s,v}$ and $\Certificate{s+1,v}$ are formed, then no higher certificate $\Certificate{s',v'}$ 
    conflicting with $\Certificate{s,v}$ can formed.
\end{lemma}

\begin{proof}
    Once $\Certificate{s+1,v}$ extending $\Certificate{s,v}$ is formed, it implies that at 
    least $\f+1$ correct replicas lock on $\Certificate{s,v}$ at slot $s$ of view $v$. The $f+1$ correct 
    replicas would not vote for blocks conflicting with $B_{s,v}$ in higher slots and views. Then, no 
    higher certificate $\Certificate{s',v'}$ conflicting with $\Certificate{s,v}$ can be formed.
\end{proof}

\begin{lemma} \label{lm2:no-gap-rule-2}
    If block $B_{s^{*},v^{*}}$ is directly extended by block $B_{1,v}$ and certificate
    $\Certificate{1,v}$ is formed and \MName{NewView} certificate $\Certificate{s^{*},v^{*}}$ is formed, then no higher certificate $\Certificate{s',v'}$ 
    conflicting with $\Certificate{s^{*},v^{*}}$ can formed.
\end{lemma}

\begin{proof}
    If \MName{NewView} certificate $\Certificate{s^{*},v^{*}}$ is formed, then it means at least $\f+1$ correct replicas did not vote for any conflicting block between 
    $B_{s^*, v^*}$ and $B_{1,v}$. Thus, no conflicting certificate $\Certificate{s',v'}$ between $B_{s^*, v^*}$ and $B_{1,v}$ can be formed.
    
    $\Certificate{1,v}$ implies that at least $\f+1$ correct replicas lock on $\Certificate{s^*,v^*}$ at view $v$. then no  certificate $\Certificate{s',v'}$ 
    conflicting with $\Certificate{s^{*},v^{*}}$ and higher than $B_{1,v}$ can formed.

    In summary, no higher certificate $\Certificate{s',v'}$ 
    conflicting with $\Certificate{s^{*},v^{*}}$ can formed.
\end{proof}

\begin{lemma}\label{lm2:certificate}
    If a correct replica $R$ commits a block $B_{s_v,v}$, then no other block can cause it to be rollbacked.
\end{lemma}

\begin{proof}
    Let block $B_{s_w,w}, w > v$ be a block that conflicts with block $B_{s_v,v}$, and assume that another correct replica $R'$ commits $B_{s_w,w}$.
    This implies that replicas $R$ and $R'$ have conflicting global-ledgers.
    For both blocks $B_{s_v,v}$ and $B_{s_w,w}$ to commit, $R$ and $R'$ must have received a 
    no-gap-extension certificate pairs $P_v$ and $P_w$, respectively, where $P_i, i = {v,w}$, represent a \emph{no-gap-extension} certificate pair as described in Lemma~\ref{lm2:no-gap-rule} and Lemma~\ref{lm2:no-gap-rule-2}.
    
    If $P_1$ is lower than $P_2$, from Lemma~\ref{lm2:no-gap-rule} and Lemma~\ref{lm2:no-gap-rule-2}, we know that once $P_1$ formed, then it is impossible to form $P_2$. 
    Thus, it contradicts the fact that $B_{s_w,w}$ is committed by $R'$.

    If $P_2$ is lower than $P_1$, from Lemma~\ref{lm2:no-gap-rule} and Lemma~\ref{lm2:no-gap-rule-2}, we know that once $P_2$ formed, then it is impossible to form $P_1$. 
    Thus, it contradicts the fact that $B_{s_v,v}$ is committed by $R$.

    Therefore, we know that the assumption that $R'$ commits $B_{s_w,w}$ cannot hold, 
    and then no other block can cause $B_{s_v,v}$ to be rollbacked.
\end{proof}

\begin{theorem}\label{thm2:safety}
    (Safety) \PHSOne{} with \emph{slotting} guarantees a safe consensus in a system of $n \ge 3\f+1$.
    % \Sadoghi{this is the only theorem that references HS.}
\end{theorem}

\begin{proof}
    Using Lemma~\ref{prop2:non_divergent}, we proved that in \PHSOne{} with \emph{slotting}, no two correct replicas 
    will execute different blocks for the same slot. Further, using Lemma~\ref{lm2:certificate}, 
    we show that no two correct replicas can commit conflicting blocks. Consequently, this allows us to claim that \PHSOne{} with \emph{slotting} guarantees safety.
\end{proof}

\begin{lemma}\label{lemma2:uniquebranch}
If $\f+1$ correct replicas speculatively execute $B_{s,v}$ client responses, 
then no higher conflicting certificate can be formed.
\end{lemma}

\begin{proof}
% If $\f+1$ correct replicas speculatively execute $B_v$.  then in view $v+1$, 
% such $\f+1$ correct replicas receive and lock on $\Certificate{v}$. Thus, for 
% any higher conflicting proposal, there are at most $2\f < \n-\f$ votes. 
% Thus, no higher conflicting certificate can be formed.
Similar to the proof of Lemma~\ref{lemma:uniquebranch}.

\end{proof}

\begin{lemma}\label{lemma2:noconflictcommit}
If a client receives $\n-\f$ responses for block $B_{s,v}$, then no higher 
conflicting block can be committed.
\end{lemma}

\begin{proof}
% With the \emph{Prefix Speculation Rule}, we know that in \\\PHSOne{}, there are 
% only two cases in which a correct replica $R$ sends a response for a block $B_v$: 
% (1) $R$ commits $B_v$; (2) In view $v+1$, $R$ speculatively executes $B_v$.

% Among the $\n-\f$ responses, there are $\f+1$ correct responses from correct replicas. 
% If all of the $\f+1$ correct responses are speculative responses, then from 
% Lemma~\ref{lemma:uniquebranch} we know that no higher conflicting certificate can be 
% formed, and no higher conflicting block can be committed. If any of the $\f+1$ correct 
% responses is not a speculative response, then one correct replica has committed $B_v$. 
% From Theorem~\ref{thm:safety}, we know that no conflicting block can be committed.
Similar to the proof of Lemma~\ref{lemma:noconflictcommit}.
\end{proof}

% % \begin{proof}
% %     Using Lemma~\ref{prop:non_divergent}, we proved that in \PHSOne{}, no two correct replicas 
% %     will execute different blocks for the same view. Further, using Lemma~\ref{lm:certificate}, 
% %     we show that no two correct replicas can commit conflicting blocks. Consequently, this allows 
% %     us to claim that \PHSOne{} guarantees safety.
% % \end{proof}

% \begin{lemma}\label{lm2:viewlength}
%     If a correct leader $\Primary{v}$ enters view $v$ at time $t > GST+\Delta$, and we set $\uptau$, 
%     the length of view $v$, to be $\uptau > 5\Delta$, then $\Primary{v}$ can form $\Certificate{v}$.
% \end{lemma}

% \begin{proof}
%     The \emph{pacemaker} protocol ensures that all correct replicas enter view $v$ 
%     before $t+2\Delta$. If $\Primary{v}$ does not learn about $\Certificate{v-1}$, then 
%     it receives the \emph{highest certificate} from correct replicas by $t+3\Delta$
%     and then broadcasts \MName{Propose} message for $B_v$. Otherwise, $\Primary{v}$ 
%     broadcasts \MName{Propose} message $m$ for $B_v$ directly. Then, all correct 
%     replicas receive $m$ by $t+4\Delta$. The $\Primary{v+1}$ can receive $\n-\f$ votes 
%     from correct replicas and form $\Certificate{v}$ by $t+5\Delta$.
% \end{proof}

\begin{theorem}\label{thm2:liveness}
    (Liveness) After $GST$, if we set $\uptau$, 
    the length of view $v$, to be $\uptau > 8\Delta$, correct replicas can keep \emph{committing} new blocks.
\end{theorem}

\begin{proof}
    The \emph{pacemaker} protocol ensures that all correct replicas overlap view $v$ 
    for $6\Delta$. Let's assume $t > GST$ to be the time that all correct replicas enter view $v$. 
    If $\Primary{v}$ does not form a \MName{NewView} certificate, then 
    it receives the \emph{highest certificate} from correct replicas by $t+\Delta$
    and then broadcasts \MName{Propose} message for $B_{1,v}$. Otherwise, $\Primary{v}$ 
    broadcasts \MName{Propose} message $m$ for $B_{1,v}$ directly. Then, all correct 
    replicas receive $m$ by $t+2\Delta$. The $\Primary{v}$ can receive $\n-\f$ votes 
    from correct replicas and form $\Certificate{1,v}$ by $t+3\Delta$. 
    Then, similarly, $\Primary{v}$ 
    broadcasts \MName{Propose} message $m$ for $B_{2,v}$ and forms $\Certificate{2,v}$ by $t+5\Delta$. All correct replicas receive $\Certificate{2,v}$ and commit $\Certificate{1,v}$ by $t+6\Delta$ before the view timer expires.
\end{proof}

% % \Sadoghi{The proof needs work. Are we assuming HS2 or HS3? Maybe this is an old text.}

% \begin{proof}
%     Based on Lemma~\ref{lm:viewlength}, we know that after \emph{GST}, if there are 
%     three consecutive correct leaders $\Primary{v}, \Primary{v+1}, \Primary{v+2}$, 
%     then $\Certificate{v}$ and $\Certificate{v+1}$ can be formed and seen by all 
%     correct replicas; thus, $B_v$ satisfies the \emph{Commit Rule} for all 
%     correct replicas. Since there are at most $\f$ faulty replicas out of the 
%     $3\f+1$ replicas, it is for sure that there are three consecutive correct 
%     leaders as we rotate leaders in a round-robin way. Then, correct replicas 
%     can keep \emph{committing} new blocks.
% \end{proof}

\begin{corollary}
If a client receives $\n-\f$ responses for block $B_v$, then $B_v$ will eventually 
be committed by correct replicas.
\end{corollary}

\begin{proof}
Similar to the proof of Corollary~\ref{crly:response}.
\end{proof}



% % \Sadoghi{There is no mention of our commit rules, which will probably replace 
% % these directly and certainly execute verbiage.}


